Sound, Fine-Grained Traversal Fusion for Heterogeneous Trees - Extended Version

Applications in many domains are based on a series of traversals of tree structures, and fusing these traversals together to reduce the total number of passes over the tree is a common, important optimization technique. In applications such as compilers and render trees, these trees are heterogeneous: different nodes of the tree have different types. Unfortunately, prior work for fusing traversals falls short in different ways: they do not handle heterogeneity; they require using domain-specific languages to express an application; they rely on the programmer to aver that fusing traversals is safe, without any soundness guarantee; or they can only perform coarse-grain fusion, leading to missed fusion opportunities. This paper addresses these shortcomings to build a framework for fusing traversals of heterogeneous trees that is automatic, sound, and fine-grained. We show across several case studies that our approach is able to allow programmers to write simple, intuitive traversals, and then automatically fuse them to substantially improve performance.

==> __latexindent_temp.tex <==
@article{wadler1990,
title = "Deforestation: transforming programs to eliminate trees",
journal = "Theoretical Computer Science",
volume = "73",
number = "2",
pages = "231 - 248",
year = "1990",
issn = "0304-3975",
doi = "https://doi.org/10.1016/0304-3975(90)90147-A",
url = "http://www.sciencedirect.com/science/article/pii/030439759090147A",
author = "Philip Wadler"
}

@article{johann2002,
author="Johann, Patricia",
title="A Generalization of Short-Cut Fusion and its Correctness Proof",
journal="Higher-Order and Symbolic Computation",
year="2002",
month="Dec",
day="01",
volume="15",
number="4",
pages="273--300",
abstract="Short-cut fusion is a program transformation technique that uses a single, local transformation---called the foldr-build rule---to remove certain intermediate lists from modularly constructed functional programs. Arguments that short-cut fusion is correct typically appeal either to intuition or to ``free theorems''---even though the latter have not been known to hold for the languages supporting higher-order polymorphic functions and fixed point recursion in which short-cut fusion is usually applied. In this paper we use Pitts' recent demonstration that contextual equivalence in such languages is relationally parametric to prove that programs in them which have undergone short-cut fusion are contextually equivalent to their unfused counterparts. For each algebraic data type we then define a generalization of build which constructs substitution instances of its associated data structures, and use Pitts' techniques to prove the correctness of a contextual equivalence-preserving fusion rule which generalizes short-cut fusion. These rules optimize compositions of functions that uniformly consume algebraic data structures with functions that uniformly produce substitution instances of those data sructures.",
issn="1573-0557",
doi="10.1023/A:1022982420888",
url="https://doi.org/10.1023/A:1022982420888"
}

@article{sakka2017,
 author = {Sakka, Laith and Sundararajah, Kirshanthan and Kulkarni, Milind},
 title = {TreeFuser: A Framework for Analyzing and Fusing General Recursive Tree Traversals},
 journal = {Proc. ACM Program. Lang.},
 issue_date = {October 2017},
 volume = {1},
 number = {OOPSLA},
 month = oct,
 year = {2017},
 issn = {2475-1421},
 pages = {76:1--76:30},
 articleno = {76},
 numpages = {30},
 url = {http://doi.acm.org/10.1145/3133900},
 doi = {10.1145/3133900},
 acmid = {3133900},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Fusion, Locality Optimization, Recursive Tree Traversals},
} 

@article{chin1999fusiontupling,
author = {Chin, Wei-ngan and Hu, Zhenjiang and Takeichi, Masato},
year = {1999},
month = {12},
pages = {},
title = {A Modular Derivation Strategy via Fusion and Tupling}
}

@article{chin1994fusion, 
title={Safe fusion of functional expressions II: Further improvements}, 
volume={4}, 
DOI={10.1017/S0956796800001179}, 
number={4}, 
journal={Journal of Functional Programming}, 
publisher={Cambridge University Press}, 
author={Chin, Wei-Ngan}, 
year={1994}, 
pages={515–555}
}

@inproceedings{arkel2003fusion,
 author = {Van Arkel, Diederik and Van Groningen, John and Smetsers, Sjaak},
 title = {Fusion in Practice},
 booktitle = {Proceedings of the 14th International Conference on Implementation of Functional Languages},
 series = {IFL'02},
 year = {2003},
 isbn = {3-540-40190-3},
 location = {Madrid, Spain},
 pages = {51--67},
 numpages = {17},
 url = {http://dl.acm.org/citation.cfm?id=1756972.1756976},
 acmid = {1756976},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 

@inproceedings{chin1993tuple,
 author = {Chin, Wei-Ngan},
 title = {Towards an Automated Tupling Strategy},
 booktitle = {Proceedings of the 1993 ACM SIGPLAN Symposium on Partial Evaluation and Semantics-based Program Manipulation},
 series = {PEPM '93},
 year = {1993},
 isbn = {0-89791-594-1},
 location = {Copenhagen, Denmark},
 pages = {119--132},
 numpages = {14},
 url = {http://doi.acm.org/10.1145/154630.154643},
 doi = {10.1145/154630.154643},
 acmid = {154643},
 publisher = {ACM},
 address = {New York, NY, USA},
}
 
@inproceedings{chin1995fusiontupling,
  title={Fusion and tupling transformations: Synergies and conflicts},
  author={Chin, W},
  booktitle={Proceedings of the Fuji International Workshop on Functional and Logic Programming, Susono, Japan},
  pages={106--125},
  year={1995},
  organization={World Scientific Publishing}
}
@InProceedings{vollmer2017,
  author =	{Michael Vollmer and Sarah Spall and Buddhika Chamith and Laith Sakka and Chaitanya Koparkar and Milind Kulkarni and Sam Tobin-Hochstadt and Ryan R. Newton},
  title =	{{Compiling Tree Transforms to Operate on Packed Representations}},
  booktitle =	{31st European Conference on Object-Oriented Programming (ECOOP 2017)},
  pages =	{26:1--26:29},
  series =	{Leibniz International Proceedings in Informatics (LIPIcs)},
  ISBN =	{978-3-95977-035-4},
  ISSN =	{1868-8969},
  year =	{2017},
  volume =	{74},
  editor =	{Peter M{\"u}ller},
  publisher =	{Schloss Dagstuhl--Leibniz-Zentrum fuer Informatik},
  address =	{Dagstuhl, Germany},
  URL =		{http://drops.dagstuhl.de/opus/volltexte/2017/7273},
  URN =		{urn:nbn:de:0030-drops-72737},
  doi =		{10.4230/LIPIcs.ECOOP.2017.26},
  annote =	{Keywords: compiler optimization, program transformation, tree traversal}
}

@inproceedings{petrashko2017,
 author = {Petrashko, Dmitry and Lhot\'{a}k, Ond\v{r}ej and Odersky, Martin},
 title = {Miniphases: Compilation Using Modular and Efficient Tree Transformations},
 booktitle = {Proceedings of the 38th ACM SIGPLAN Conference on Programming Language Design and Implementation},
 series = {PLDI 2017},
 year = {2017},
 isbn = {978-1-4503-4988-8},
 location = {Barcelona, Spain},
 pages = {201--216},
 numpages = {16},
 url = {http://doi.acm.org/10.1145/3062341.3062346},
 doi = {10.1145/3062341.3062346},
 acmid = {3062346},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {cache locality, compiler performance, tree traversal fusion},
}

@inproceedings{rajbhandari2016a,
 author = {Rajbhandari, Samyam and Kim, Jinsung and Krishnamoorthy, Sriram and Pouchet, Louis-No\"{e}l and Rastello, Fabrice and Harrison, Robert J. and Sadayappan, P.},
 title = {On Fusing Recursive Traversals of K-d Trees},
 booktitle = {Proceedings of the 25th International Conference on Compiler Construction},
 series = {CC 2016},
 year = {2016},
 isbn = {978-1-4503-4241-4},
 location = {Barcelona, Spain},
 pages = {152--162},
 numpages = {11},
 url = {http://doi.acm.org/10.1145/2892208.2892228},
 doi = {10.1145/2892208.2892228},
 acmid = {2892228},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Tree traversal, data locality, fusion},
} 

@inproceedings{rajbhandari2016b,
 author = {Rajbhandari, Samyam and Kim, Jinsung and Krishnamoorthy, Sriram and Pouchet, Louis-Noel and Rastello, Fabrice and Harrison, Robert J. and Sadayappan, P.},
 title = {A Domain-specific Compiler for a Parallel Multiresolution Adaptive Numerical Simulation Environment},
 booktitle = {Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis},
 series = {SC '16},
 year = {2016},
 isbn = {978-1-4673-8815-3},
 location = {Salt Lake City, Utah},
 pages = {40:1--40:12},
 articleno = {40},
 numpages = {12},
 url = {http://dl.acm.org/citation.cfm?id=3014904.3014958},
 acmid = {3014958},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
} 
@inproceedings{meyerovich2010,
	Acmid = {1772763},
	Address = {New York, NY, USA},
	Author = {Meyerovich, Leo A. and Bodik, Rastislav},
	Booktitle = {Proceedings of the 19th International Conference on World Wide Web},
	Doi = {10.1145/1772690.1772763},
	Isbn = {978-1-60558-799-8},
	Keywords = {attribute grammar, box model, css, font, html, layout, mobile, multicore, selector},
	Location = {Raleigh, North Carolina, USA},
	Numpages = {10},
	Pages = {711--720},
	Publisher = {ACM},
	Series = {WWW '10},
	Title = {Fast and Parallel Webpage Layout},
	Url = {http://doi.acm.org/10.1145/1772690.1772763},
	Year = {2010},
	Bdsk-Url-1 = {http://doi.acm.org/10.1145/1772690.1772763},
	Bdsk-Url-2 = {http://dx.doi.org/10.1145/1772690.1772763}
}
@inproceedings{meyerovich2013,
	Acmid = {2442535},
	Address = {New York, NY, USA},
	Author = {Meyerovich, Leo A. and Torok, Matthew E. and Atkinson, Eric and Bodik, Rastislav},
	Booktitle = {Proceedings of the 18th ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming},
	Doi = {10.1145/2442516.2442535},
	Isbn = {978-1-4503-1922-5},
	Keywords = {attribute grammars, css, layout, scheduling, sketching},
	Location = {Shenzhen, China},
	Numpages = {10},
	Pages = {187--196},
	Publisher = {ACM},
	Series = {PPoPP '13},
	Title = {Parallel Schedule Synthesis for Attribute Grammars},
	Url = {http://doi.acm.org/10.1145/2442516.2442535},
	Year = {2013},
	Bdsk-Url-1 = {http://doi.acm.org/10.1145/2442516.2442535},
	Bdsk-Url-2 = {http://dx.doi.org/10.1145/2442516.2442535}
  }

 @phdthesis{nanopass,
 author = {Sarkar, Dipanwita},
 advisor = {Dybvig, R. Kent},
 title = {Nanopass Compiler Infrastructure},
 year = {2008},
 isbn = {978-0-549-91996-4},
 note = {AAI3337263},
 publisher = {Indiana University},
 address = {Indianapolis, IN, USA},
} 

@Inproceedings{openfst,
author={Allauzen, Cyril and Riley, Michael and Schalkwyk, Johan and Skut, Wojciech and Mohri, Mehryar},
title={OpenFst: A General and Efficient Weighted Finite-State Transducer Library},
booktitle={Implementation and Application of Automata},
year={2007},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={11--23},
isbn={978-3-540-76336-9}
}

@article{Chilimbi1999,
  author =        {Chilimbi, TM and Hill, MD and Larus, JR},
  journal =       {ACM SIGPLAN Notices},
  title =         {{Cache-conscious structure layout}},
  year =          {1999},
  annote =        {This is the ccmorph paper.},
  url =           {http://dl.acm.org/citation.cfm?id=301633},
}

@inproceedings{Truong1998,
  address =       {Washington, DC, USA},
  author =        {Truong, D. N. and Bodin, F. and Seznec, A.},
  booktitle =     {Proceedings of the 1998 International Conference on
                   Parallel Architectures and Compilation Techniques},
  pages =         {322--},
  publisher =     {IEEE Computer Society},
  series =        {PACT '98},
  title =         {Improving Cache Behavior of Dynamically Allocated
                   Data Structures},
  year =          {1998},
  isbn =          {0-8186-8591-3},
  url =           {http://portal.acm.org/citation.cfm?id=522344.825680},
}

@article{Lattner2005,
  author =        {Lattner, Chris and Adve, Vikram},
  journal =       {ACM SIGPLAN Notices},
  pages =         {129--142},
  title =         {{Automatic pool allocation: improving performance by
                   controlling data structure layout in the heap}},
  volume =        {40},
  year =          {2005},
  abstract =      {This paper describes Automatic Pool Allocation, a
                   transformation framework that segregates distinct
                   instances of heap-based data structures into seperate
                   memory pools and allows heuristics to be used to
                   partially control the internal layout of those data
                   structures. The primary goal of this work is
                   performance improvement, not automatic memory
                   management, and the paper makes several new
                   contributions. The key contribution is a new compiler
                   algorithm for partitioning heap objects in imperative
                   programs based on a context-sensitive pointer
                   analysis, including a novel strategy for correct
                   handling of indirect (and potentially unsafe)
                   function calls. The transformation does not require
                   type safe programs and works for the full generality
                   of C and C++. Second, the paper describes several
                   optimizations that exploit data structure
                   partitioning to further improve program performance.
                   Third, the paper evaluates how memory hierarchy
                   behavior and overall program performance are impacted
                   by the new transformations. Using a number of
                   benchmarks and a few applications, we find that
                   compilation times are extremely low, and overall
                   running times for heap intensive programs speed up by
                   10-25\% in many cases, about 2x in two cases, and
                   more than 10x in two small benchmarks. Overall, we
                   believe this work provides a new framework for
                   optimizing pointer intensive programs by segregating
                   and controlling the layout of heap-based data
                   structures.},
  annote =        {Looks very apt. Also a good seed for pulling in the
                   region inference literature. (MLKit being the obvious
                   one)},
  doi =           {10.1145/1065010.1065027},
  isbn =          {1595930566},
  issn =          {0362-1340},
}


@misc{Chilimbi1999a,
  author =        {Chilimbi, Trishul M. and Larus, James R.},
  booktitle =     {ACM SIGPLAN Notices},
  pages =         {37--48},
  title =         {{Using generational garbage collection to implement
                   cache-conscious data placement}},
  volume =        {34},
  year =          {1999},
  abstract =      {Processor and memory technology trends show a
                   continual increase in the cost of accessing main
                   memory. Machine designers have tried to mitigate the
                   effect of this trend through a variety of techniques
                   that attempt to reduce or tolerate memory latency.
                   These techniques, unfortunately, have only been
                   partially successful for pointer- manipulating
                   programs. Recent research has demonstrated that these
                   programs can benefit greatly from the complementary
                   approach of reorganizing pointer data structures to
                   improve cache locality. This paper describes how a
                   generational garbage collector can be used to achieve
                   a cache-conscious data layout, in which objects with
                   high temporal affinity are placed next to each other,
                   so they are likely to reside in the same cache block.
                   The paper demonstrates the feasibility of collecting
                   low overhead, real-time profiling information about
                   data access patterns for object-oriented languages,
                   and describes a new copying algorithm that utilizes
                   this information to produce a cache-conscious object
                   layout. Preliminary results indicate that this
                   technique reduces cache miss rates by
                   21-42$\backslash$\%, and improves program performance
                   by 14-37$\backslash$\%.},
  doi =           {10.1145/301589.286865},
  isbn =          {1-58113-114-3},
  issn =          {03621340},
}


@inproceedings{stream-fusion,
 author = {Coutts, Duncan and Leshchinskiy, Roman and Stewart, Don},
 title = {Stream Fusion: From Lists to Streams to Nothing at All},
 booktitle = {Proceedings of the 12th ACM SIGPLAN International Conference on Functional Programming},
 series = {ICFP '07},
 year = {2007},
 isbn = {978-1-59593-815-2},
 location = {Freiburg, Germany},
 pages = {315--326},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/1291151.1291199},
 doi = {10.1145/1291151.1291199},
 acmid = {1291199},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {deforestation, functional programming, program fusion, program optimisation, program transformation},
}
@inproceedings{weijiang15,
 author = {Weijiang, Yusheng and Balakrishna, Shruthi and Liu, Jianqiao and Kulkarni, Milind},
 title = {Tree Dependence Analysis},
 booktitle = {Proceedings of the 36th ACM SIGPLAN Conference on Programming Language Design and Implementation},
 series = {PLDI '15},
 year = {2015},
 isbn = {978-1-4503-3468-6},
 location = {Portland, OR, USA},
 pages = {314--325},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2737924.2737972},
 doi = {10.1145/2737924.2737972},
 acmid = {2737972},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {dependence analysis, irregular algorithms, loop transformations},
}




@inproceedings{emami94,
 author = {Emami, Maryam and Ghiya, Rakesh and Hendren, Laurie J.},
 title = {Context-sensitive Interprocedural Points-to Analysis in the Presence of Function Pointers},
 booktitle = {Proceedings of the ACM SIGPLAN 1994 Conference on Programming Language Design and Implementation},
 series = {PLDI '94},
 year = {1994},
 isbn = {0-89791-662-X},
 location = {Orlando, Florida, USA},
 pages = {242--256},
 numpages = {15},
 url = {http://doi.acm.org/10.1145/178243.178264},
 doi = {10.1145/178243.178264},
 acmid = {178264},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{hegde17ispass, 
author={Nikhil Hegde and Jianqiao Liu and Kirshanthan Sundararajah and Milind Kulkarni}, 
booktitle={2017 IEEE International Symposium on Performance Analysis of Systems and Software (ISPASS)}, 
title={Treelogy: A benchmark suite for tree traversals}, 
year={2017}, 
pages={227-238}, 
keywords={distributed memory systems;graphics processing units;ontologies (artificial intelligence);optimisation;shared memory systems;trees (mathematics);GPU;Treelogy;algorithmic kernels;attributes extraction;benchmark suite;distributed memory systems;ontology;optimizations;shared memory multicores;structural properties;tree traversals;Algorithm design and analysis;Benchmark testing;Correlation;Data mining;Kernel;Ontologies;Optimization}, 
doi={10.1109/ISPASS.2017.7975294}, 
month={April},}
